The simplest scoto-seesaw model: WIMP dark matter phenomenology and Higgs vacuum stability

We analyze the consistency of electroweak breaking, neutrino and dark matter phenomenology within the simplest scoto-seesaw model. By adding the minimal dark sector to the simplest "missing partner" type-I seesaw one has a physical picture for the neutrino oscillation lengths: the "atmospheric" mass scale arises from the tree-level seesaw, while the "solar" scale is induced radiatively, mediated by the dark sector. We identify parameter regions consistent with theoretical constraints, as well as dark matter relic abundance and direct detection searches. Using two-loop renormalization group equations we explore the stability of the vacuum and the consistency of the underlying dark parity symmetry. One also has a lower bound for the neutrinoless double beta decay amplitude.

==> Makefile <==
FILENAME=Scotogenic_June
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = Scotogenic_June.ps 
PDFFILE = Scotogenic_June.pdf

COPY = if test -r Scotogenic_June.toc; then cp Scotogenic_June.toc Scotogenic_June.toc.bak; fi 
RM = /bin/rm -f

CLEAN=rm -f Scotogenic_June.aux Scotogenic_June.log Scotogenic_June.dvi Scotogenic_June.toc Scotogenic_June.out Scotogenic_June.blg Scotogenic_June.mtc Scotogenic_June.mtc1 Scotogenic_June.rel Scotogenic_June.vrb Scotogenic_June.end Scotogenic_June.spl *.aux *~ \#*

WARNING=egrep -i "(Reference|Citation).*undefined" Scotogenic_June.log ; true

HELP=cat /home/jv/bin/help/MakePDFLatexMakefile.help

main:	Scotogenic_June.tex pdf

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	PhysBiblio.exe tex bibliography.bib './Response/response.tex' './Scotogenic_June.tex' 
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl

help:
	$(HELP)

complete: realclean pdf clean


